A Survey on Decentralized Identifiers and Verifiable Credentials

Digital identity has always been considered the keystone for implementing secure and trustworthy communications among parties. The ever-evolving digital landscape has gone through many technological transformations that have also affected the way entities are digitally identified. During this digital evolution, identity management has shifted from centralized to decentralized approaches. The last era of this journey is represented by the emerging Self-Sovereign Identity (SSI), which gives users full control over their data. SSI leverages decentralized identifiers (DIDs) and verifiable credentials (VCs), which have been recently standardized by the World Wide Web Community (W3C). These technologies have the potential to build more secure and decentralized digital identity systems, remarkably contributing to strengthening the security of communications that typically involve many distributed participants. It is worth noting that the scope of DIDs and VCs extends beyond individuals, encompassing a broad range of entities including cloud, edge, and Internet of Things (IoT) resources. However, due to their novelty, existing literature lacks a comprehensive survey on how DIDs and VCs have been employed in different application domains, which go beyond SSI systems. This paper provides readers with a comprehensive overview of such technologies from different perspectives. Specifically, we first provide the background on DIDs and VCs. Then, we analyze available implementations and offer an in-depth review of how these technologies have been employed across different use-case scenarios. Furthermore, we examine recent regulations and initiatives that have been emerging worldwide. Finally, we present some challenges that hinder their adoption in real-world scenarios and future research directions.

==> sections/lesson.tex <==
\section{Lessons Learned}\label{lessons}
DIDs and VCs have experienced a surge in popularity only in recent years, which means that research in this area is still in its infancy. In the following section, we highlight the key insights gained during the development of the core sections of this survey.

\subsection{Implementations}

\subsection{Applications}
By reviewing the existing body of research, it becomes evident that DIDs and VCs have found application in a wide variety of fields, which apparently may not have much in common such as smart transportation and smart healthcare. What unites these seemingly distinct domains is the fact that these technologies are frequently harnessed as key components in the implementation of SSI systems. This lies in their ability to empower individuals with complete control over their data, enabling them to selectively share information. As a result, communications will be more secure and potential data breaches will be mitigated, fostering a safer digital landscape. Moreover, as underscored by the diverse application domains, these decentralized identities can be utilized across a multitude of platforms and applications, thereby favoring interoperability and improving user experience. For example, let us consider the versatility of a VC, which can seamlessly facilitate access to both educational and healthcare services.

However, although existing literature primarily focuses on DIDs and VCs as building blocks for SSI systems, their usage can be also extended to fulfill the stringent demands of all the applications necessitating secure and verifiable identity credentials. For instance, in the landscape of smart supply chains, DIDs 
can be used to track operations, whereas VCs are employed to prove the process is adhering to certain requirements. In this case, VCs effectively serve as certificates, thus their role emphasizes decentralized verification more than the selective disclosure of information.  

\subsection{Regulations}



==> sections/related.tex <==



==> sections/summaryfeatures.tex <==
\section{Main Features of DIDs and VCs}\label{summary}
The comprehensive examination of existing literature on DIDs and VCs, coupled with the analysis of emerging regulations and initiatives worldwide, underscores the crucial role these emerging standards play in shaping both the current and future digital identity landscapes. This section presents the main features of DIDs and VCs.

\subsection{DID Features}

\begin{enumerate}
    \item \emph{Self-Sovereignty}: Users have control and ownership over their DIDs, which can be created and managed by themselves. This self-sovereignty makes individuals independent from central authorities or third-party entities.
    \item \emph{Inclusivity}: DIDs facilitate inclusivity by providing digital access to individuals in least-developed countries lacking traditional forms of identification such as government-issued IDs.
    \item \emph{Privacy and Security}: DIDs allow users to selectively disclose information, preventing the oversharing of personal data. Employing cryptographic techniques like PKI for key generation, digital signature, and encryption, DIDs ensure robust defenses against unauthorized access and data breaches. Additionally, the use of decentralized networks such as DLT reduces the risk of a single point of failure, enhancing overall security.
    \item \emph{Interoperability and Portability}: DIDs are designed to be compatible with various platforms, fostering seamless integration and communication across different systems. Moreover, they promote portability by enabling users to easily transfer their identifiers and associated data across various platforms.
    \item \emph{Persistence}: DIDs are consistent and permanent, offering a reliable means of identification even as individuals switch service providers or platforms.
\end{enumerate}

%In the following, we summarize the key features of VCs:

\subsection{VC Features}

\begin{enumerate}
    \item \emph{Decentralized Verification}:  Entities issuing VCs are inherently trusted, ensuring reliable verification of credential authenticity and contained information. VCs can be verified independently at any location and time without direct interaction with the issuer. 
    \item \emph{Privacy and Security}: VCs support ZKP and selective disclosure, granting users the autonomy to share only necessary information with verifiers, without compromising entire credentials. Personal information is not stored on Distributed Ledger Technologies DLTs or centralized systems, minimizing the risk of data breaches. Moreover, by providing data owners full control over their data, VCs can help organizations become compliant with existing regulations such as the GDPR.
    \item \emph{Interoperability and Portability}: W3C standards promote a standardized approach to VC implementation, ensuring high interoperability and consistency. VCs are designed to seamlessly operate across different platforms and applications. Individuals can store VCs in their digital wallet and take them anywhere while still being verifiable, offering users flexibility and convenience in presenting their credentials.
    \item \emph{Temper-Resistance}: VCs are cryptographically signed, making them resistant to tampering or unauthorized alterations, thereby ensuring the integrity of the information included.
\end{enumerate}

